Grid-Based Decimation for Wavelet Transforms with Stably Invertible Implementation

The constant center frequency to bandwidth ratio (Q-factor) of wavelet transforms provides a very natural representation for audio data. However, invertible wavelet transforms have either required non-uniform decimation -- leading to irregular data structures that are cumbersome to work with -- or require excessively high oversampling with unacceptable computational overhead. Here, we present a novel decimation strategy for wavelet transforms that leads to stable representations with oversampling rates close to one and uniform decimation. Specifically, we show that finite implementations of the resulting representation are energy-preserving in the sense of frame theory. The obtained wavelet coefficients can be stored in a timefrequency matrix with a natural interpretation of columns as time frames and rows as frequency channels. This matrix structure immediately grants access to a large number of algorithms that are successfully used in time-frequency audio processing, but could not previously be used jointly with wavelet transforms. We demonstrate the application of our method in processing based on nonnegative matrix factorization, in onset detection, and in phaseless reconstruction.

==> header.tex <==
\usepackage{amsmath,amssymb,amsthm,amsfonts,amsopn,cite,mathrsfs,todonotes}
\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{ifpdf}
\usepackage[english]{babel}
%\usepackage{subfig} 
\usepackage[ruled]{algorithm2e}
%\usepackage{hyperref}
%\usepackage[notref,notcite]{showkeys}
\usepackage{dsfont,url}
\usepackage{tikz}
\usepackage{multirow}
\usetikzlibrary{patterns}
\usetikzlibrary{calc}
\usetikzlibrary{arrows.meta}
\usepackage{graphicx}



\newcounter{tempEquationCounter}
\newcounter{thisEquationNumber}
\newenvironment{floatEq}
{\setcounter{thisEquationNumber}{\value{equation}}\addtocounter{equation}{1}
%record equation as happened and remember number
\begin{figure*}[tb]% float following equation across columns
\hrulefill\vspace*{4pt}
\normalsize\setcounter{tempEquationCounter}{\value{equation}}
% record current equation number in floated location
\setcounter{equation}{\value{thisEquationNumber}}% use previous equation number
}
{\setcounter{equation}{\value{tempEquationCounter}}
% set back to equation number in floated location
\hrulefill\vspace*{-1em}% add a horizontal rule separator
\end{figure*}% end float environment
}



\theoremstyle{plain}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}{Definition}%[section]
\newtheorem{assumption}{Assumption}%[section]
\theoremstyle{remark}
\newtheorem{remark}{Remark}%[section]
\newtheorem{example}{Example}%[section]
\theoremstyle{remark}
\newtheorem*{rem*}{Remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%% TeX-macros %%%%%%%%%
%%
%\numberwithin{equation}{section}

\newcommand{\bd}{\mathbf}   
% \newcommand{\abs}[1]{\lvert#1\rvert}   %big absolute value
\renewcommand{\mod}{\mathop{\operatorname{mod}}}  
\newcommand{\vol}{\mathop{\operatorname{vol}}}
\newcommand{\LtR}{\mathbf L^2(\mathbb{R})}
\newcommand{\LtRd}{\mathbf L^2(\mathbb{R}^d)}
\newcommand{\LiR}{\mathbf L^1(\mathbb{R})}
\newcommand{\LiRd}{\mathbf L^1(\mathbb{R^d})}

\newcommand{\FF}{\mathcal F}

\newcommand{\RR}{\mathbb R}
\newcommand{\ZZ}{\mathbb Z}
\newcommand{\NN}{\mathbb N}
\newcommand{\CC}{\mathbb C}

\def\supp{\mathop{\operatorname{supp}}}
\def\sgn{\mathop{\operatorname{sgn}}}

\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}
\DeclareMathAccent{\widecheck}{0}{mathx}{"71}
\DeclareMathAccent{\wideparen}{0}{mathx}{"75}
\newcommand{\grad}{\nabla}
\newcommand{\Indicator}{{\mathds{1}}}
\newcommand{\modulation}{\bd{M}}
\newcommand{\translation}{\bd{T}}
\newcommand{\lebesgue}{\bd{L}}
\newcommand{\continuous}{{\mathcal{C}}}
\newcommand{\Fourier}{\mathcal{F}}

\newcommand{\Glg}{{\mathcal G(\gamma,g)}}
\newcommand{\GlTg}{{\mathcal G(\gamma,\bd T g)}}
\newcommand{\GlDg}{{\mathcal G(\gamma,g')}}
\newcommand{\GlTtg}{{\mathcal G(\gamma,\bd T^2 g)}}
\newcommand{\GlTDg}{{\mathcal G(\gamma,\bd T g')}}
\newcommand{\Glgn}{{\mathcal G(\gamma,g_0)}}
\newcommand{\GlTgn}{{\mathcal G(\gamma,\bd T g_0)}}
\newcommand{\GlDgn}{{\mathcal G(\gamma,g_0')}}
\newcommand{\GlTtgn}{{\mathcal G(\gamma,\bd T^2 g_0)}}
\newcommand{\GlTDgn}{{\mathcal G(\gamma,\bd T g_0')}}
\newcommand{\Parx}{\frac{\partial}{\partial x}}
\newcommand{\Parxt}{\frac{\partial^2}{\partial x^2}}
\newcommand{\Parxi}{\frac{\partial}{\partial \xi}}
\newcommand{\Parxit}{\frac{\partial^2}{\partial \xi^2}}
\newcommand{\Pary}{\frac{\partial}{\partial y}}
\newcommand{\Paryt}{\frac{\partial^2}{\partial y^2}}
\newcommand{\Parxy}{\frac{\partial^2}{\partial x \partial y}}

\newcommand{\gana}{g_\text{a}}
\newcommand{\gsyn}{g_\text{s}}
\newcommand{\aana}{a_\text{a}}
\newcommand{\asyn}{a_\text{s}}
\newcommand{\bana}{b_\text{a}}
\newcommand{\bsyn}{b_\text{s}}
\newcommand{\phaseana}{\phi_\text{a}}
\newcommand{\phasesyn}{\phi_\text{s}}
\newcommand{\princargg}{\text{princarg}}
\newcommand{\tgrad}{\left( \Delta_\text{t}\phi_\text{a}\right)}
\newcommand{\fgrad}{\left( \Delta_\text{s}\phi_\text{a}\right)}
\newcommand{\me}{\mathrm{e}}
\newcommand{\mi}{\mathrm{i}}
\newcommand{\princarg}[1]{\left\lbrack #1 \right\rbrack_{2\pi}}





\usepgfplotslibrary{statistics}

\pgfplotsset{
boxplot/draw/lower whisker/.style={
/pgfplots/boxplot/draw/whisker=
{\pgfplotsboxplotvalue{median}}
{\pgfplotsboxplotvalue{lower whisker}}
},
boxplot/draw/upper whisker/.style={
/pgfplots/boxplot/draw/whisker=
{\pgfplotsboxplotvalue{median}}
{\pgfplotsboxplotvalue{upper whisker}}
},
boxplot/draw/whisker/.code 2 args={
\draw [/pgfplots/boxplot/every whisker/.try]
(boxplot cs:#1) -- (boxplot cs:#2)
(boxplot whisker cs:#2,0)
--
(boxplot whisker cs:#2,0.5)
(boxplot whisker cs:#2,0.5)
--
(boxplot whisker cs:#2,1)
;
},
}

% \newif\ifpdf
% \ifx\pdfoutput\relax
% \else
%   \ifcase\pdfoutput
%       \pdffalse
%   \else
%       \pdftrue
% \fi

% \ifpdf % compiling with pdflatex
%   \pdfcompresslevel=9
%   \usepackage[pdftex]{graphicx}
% \else % compiling with latex
%   \usepackage[dvips]{epsfig,graphicx}
% \fi

\definecolor{mygreen}{RGB}{45,77,9} 
\definecolor{myred}{RGB}{255,102,102} 
\definecolor{myblue}{RGB}{105,102,255} 
\definecolor{tblblue}{rgb}{0.93,0.93,1.0}
\definecolor{tblred}{rgb}{1,0.93,0.93}
\definecolor{darkblue}{rgb}{0,0,0.5} 
\definecolor{darkgreen}{RGB}{20,120,43} 
\definecolor{darkred}{rgb}{0.8,0,0} 
\definecolor{lightblue}{RGB}{101,124,191}
\definecolor{skyblue}{RGB}{135,206,235}
\definecolor{gold}{RGB}{204,168,66}
\definecolor{strongblue}{RGB}{60,146,228}
\definecolor{lightgray}{gray}{0.5}
\definecolor{verylightgray}{RGB}{101,124,191}
\definecolor{mistyrose}{RGB}{238,213,210}
\definecolor{firebrick3}{RGB}{205,38,38}


